Measurement of the $\bar{B}_s^0\to D_s^-D_s^+$ and $\bar{B}_s^0\to D^-D_s^+$ effective lifetimes

The first measurement of the effective lifetime of the $\bar{B}_s^0$ meson in the decay $\bar{B}_s^0\to D_s^-D_s^+$ is reported using a proton-proton collision dataset, corresponding to an integrated luminosity of 3 fb$^{-1}$, collected by the LHCb experiment. The measured value of the $\bar{B}_s^0\to D_s^-D_s^+$ effective lifetime is $1.379\pm0.026\pm0.017$ ps, where the uncertainties are statistical and systematic, respectively. This lifetime translates into a measurement of the decay width of the light $\bar{B}_s^0$ mass eigenstate of \Gamma_L$=0.725\pm0.014\pm0.009$ ps$^{-1}$. The $\bar{B}_s^0$ lifetime is also measured using the flavor-specific $\bar{B}_s^0\to D^-D_s^+$ decay to be $1.52\pm0.15\pm0.01 {\rm ps}$.

==> justification.tex <==
\begin{center}
{\bf\large{Justification for Physical Review Letters}}
\end{center}

The analysis reported in this Letter is the first such measurement of the $\Bsb$ effective lifetime in $\bstodsds$
decays, and yields the most precise direct measurement of the width of the light $\Bsb$ mass eigenstate. 
The $\bstodsds$ decay is expected to be dominated by tree diagrams, and therefore the effective lifetime reported in this Letter
not only represents the most precise determination of $\GL$ in the context of the SM, its value is negligibly biased by
additional loop-mediated contributions. 
The central values of $\DGs$ and $\phi_s$ inferred from the $\Bsb$ effective lifetime measurements in $\jpsi f_0(980)$ (\CP odd)
and $\Bsb\to\Kp\Km$ (\CP even) deviate from the Standard Model expected value by about one standard deviation, and
therefore this additional, more precise measurement is of great interest.
Since larger loop contributions are expected in the $\Bsb\to\Kp\Km$ decay, precise measurements of the effective lifetimes
in $\bstodsds$ and $\Bsb\to\Kp\Km$ decays provide a complementary approach to uncovering new physics, that may affect
the latter mode but not the former. \\

\noindent {\bf Estimate word count} \\

\begin{itemize}
\item Words in text: 2676
\item Words outside text (captions, etc.): 107
\item Figures: equivalent word count (parenthesis gives aspect ratio)
 \begin{itemize} 
  \item Fig 1: 150 * 0.5  = 75
  \item Fig 2(left,right),4:  3 * 150 * (5/7) = 321
  \item Fig 3: 150 * 5/7 = 107
 \end{itemize}
\item Equations: 32 + 32 + 16 + 16 + 16 = 112
\end{itemize}

{\bf Total}: 3216 \newline

{\bf Word limit for PRL}: 3500

